The Moral Mind(s) of Large Language Models

As large language models (LLMs) increasingly participate in tasks with ethical and societal stakes, a critical question arises: do they exhibit an emergent "moral mind" - a consistent structure of moral preferences guiding their decisions - and to what extent is this structure shared across models? To investigate this, we applied tools from revealed preference theory to nearly 40 leading LLMs, presenting each with many structured moral dilemmas spanning five foundational dimensions of ethical reasoning. Using a probabilistic rationality test, we found that at least one model from each major provider exhibited behavior consistent with approximately stable moral preferences, acting as if guided by an underlying utility function. We then estimated these utility functions and found that most models cluster around neutral moral stances. To further characterize heterogeneity, we employed a non-parametric permutation approach, constructing a probabilistic similarity network based on revealed preference patterns. The results reveal a shared core in LLMs' moral reasoning, but also meaningful variation: some models show flexible reasoning across perspectives, while others adhere to more rigid ethical profiles. These findings provide a new empirical lens for evaluating moral consistency in LLMs and offer a framework for benchmarking ethical alignment across AI systems.

==> supplementary_information.tex <==

 \clearpage

 {\LARGE \  \noindent \textbf{Supplementary Information} }
 
\section{Recovering Preferences}\label{section: preferences main}

This section shows that when a model is rational, i.e., when GARP$_\mathbf{e}$ is satisfied at the highest level, $\mathbf{e=1}$, then all observed answers are maximizing a utility function. The result below draws on \cite{seror2024pricedsurveymethodologytheory}. As I will show next, the utility functions rationalizing PSM answers is singled-peaked. I define a single-peaked function as follows:
\begin{definition}\label{def: single peaked}
A function $f:X\rightarrow \mathbb{R}$ is single-peaked if
\begin{itemize}
    \item There exists a point $\mathbf{y^*}\in \mathbb{R}^S$ such that $f(\mathbf{y})\leq f(\mathbf{y^*})$ for any $\mathbf{y}\in X$.
    \item For any $\mathbf{x}, \mathbf{y} \in X$ such that $\mathbf{x}_c\leq \mathbf{y_c}\leq \mathbf{y^*_c}$ for $\mathbf{c} \in C(\mathbf{X})$, $f(\mathbf{x})\leq f(\mathbf{y})\leq f(\mathbf{y^*})$. 
\end{itemize}
\end{definition}
The second condition means that if it is possible to rank $x,y,y^*$ as $\mathbf{x_c\leq y_c\leq y^*_c}$ in a given coordinate system $c$, then $f(\mathbf{x})\leq f(\mathbf{y})$ as $\mathbf{x}$ is further away than $\mathbf{y}$ in the coordinate system $\mathbf{c}$. I define single-peaked preferences as follows:
\begin{definition}\label{Def: single peaked pref}
   A preference relation $\succcurlyeq$ is  single-peaked with respect to the order pair $(\geq, >)$ if there exists a unique $\mathbf{y}^*\in \mathbb{R}^S$ such that for any $\mathbf{x,y}\in X$, $\mathbf{x_c\leq y_c\leq y_c^*}$ for some $\mathbf{c}\in C(X)$, iif $y \succcurlyeq x$ and $\mathbf{x_c< y_c\leq y_c^*}$ iff $y \succ x$, with $\succ$ the strict part of $\succcurlyeq$. 
\end{definition}
Before turning to the Theorem, one last assumption is necessary:
\begin{assumption}
     The vertex $\mathbf{c=o^k}$ associated to round $k\in \mathcal{R}$ is the unique vertex that satisfies the condition $\mathbf{c}\leq \mathbf{q}< \mathbf{q^0_c}$ for some $\mathbf{q}\in \mathcal{B}^k$.
\end{assumption}

This assumption is made to ensure that the pre-order of the set \( X \), in round $k$, is monotonic in the coordinate system originating in \(\mathbf{o^k}\). Specifically, the assumption implies that in coordinate system originating in \(\mathbf{o^k}\), any model face a trade off between increasing the answer to one question with increasing the answer to the other questions.\footnote{Condition $\mathbf{q}< \mathbf{q^0_c}$ implies that $\mathbf{p^k.q}< \mathbf{p^k.q^0_c}$ for any $\mathbf{q}\in \mathcal{A}^r$.} Concretely, consider an example where the ideal answer is $\mathbf{q^*}=(2,2,2,2,2)$. Answer $\mathbf{q^1}=(4,4,3,2,4)$ should always be preferred to answer $\mathbf{q^2}=(5,4,5,5,5)$, because  $\mathbf{q^1}$ is closer to $(2,2,2,2,2)$ than $\mathbf{q^2}$. This can be seen by changing the coordinate system. In the coordinate system originating in $\mathbf{c}=(5,5,5,5,5)$, $\mathbf{q^1_c}=(1,1,2,3,1)$,  $\mathbf{q^2_c}=(0,1,0,0,0)$, and $\mathbf{q^*_c}=(3,3,3,3,3)$. 


A utility function $u: X\rightarrow \mathbb{R}$ weakly rationalizes the data if for all $k$ and $\mathbf{y}\in X$,  $\mathbf{p^k.q^k_{o^k}\geq p^k. y_{o^k}}$ implies that $u(\mathbf{q^k})\geq u(\mathbf{y})$. Similarly, a preference relation $\succcurlyeq$ weakly rationalizes the data iif the revealed preference pair $(R^0, P^0)$ satisfies $R^0\subset \succcurlyeq$. The following result is established by \cite{seror2024pricedsurveymethodologytheory}:
\begin{theorem}\label{theorem: halevy}
The following conditions are equivalent:
\begin{enumerate}
\item $D$ has a weak single-peaked rationalization. 
    \item The data satisfy $\text{GARP}$.

    \item There are strictly positive real numbers $U^k$ and $\lambda^k$, for each $k$ such that
    \begin{equation}\label{eq: afriat}
        U^k\leq U^l+\lambda^l \mathbf{p^l} (\mathbf{q^k_{o(l)}} - \mathbf{q^l_{o(l)}})
    \end{equation}
    for each pair of observations $(\mathbf{q^k}, \mathbf{\mathcal{B}^k}), (\mathbf{q^l}, \mathbf{\mathcal{B}^l})$ in $D$.
        \item $D$ has a single-peaked, continuous, concave utility function that rationalizes the data.
\end{enumerate}
\end{theorem}

There exists a utility function that exactly rationalizes all observed answers as utility-maximizing when GARP is satisfied. If $\mathbf{o^k=0}$ for all rounds, then Theorem \ref{theorem: halevy} is the standard version of \citeauthor{afriat1967}'s theorem. However, unlike the standard theorem, according to Theorem  \ref{theorem: halevy}, the rationalizing utility function is single-peaked rather than monotonic. This distinction offers several advantages, which will be further discussed in the application section. Briefly, single-peakedness allows us to obtain an ordinal measure of preferences that avoids the interpretational issues of traditional scale-based measures. Additionally, the peak of the utility function is defined in a continuous space, making it robust to common survey limitations such as scale bounds and order effects. Finally, using a single-peaked utility function within the PSM framework enables us to capture nuanced aspects of preferences, such as the relative importance that models assign to different survey items, thereby offering a more structured and adaptable approach to understanding moral preferences. 



==> to_delete.tex <==



estimates model-specific utility functions that best explain their responses. We found that models generally place similar weight on different moral considerations, though there are moderate variations in their ideal responses. Across the five core moral questions, most models express preferences close to neutral (2.5 on a 0–5 Likert scale), with estimated ideal responses ranging from 2.2 to 3.06. Notably, gpt-4-0125-preview exhibits slightly stronger preferences for withholding the truth and for accepting some risk of harm to a few individuals if it saves many lives, hinting at a somewhat more utilitarian moral perspective compared to other models. Additionally, comparing the estimated ideal answers to the five questions - or the peak of each model's utility - with models' responses suggest that models tend to under-report agreement with using personal data without consent for societal benefits, restricting individual autonomy for the sake of collective welfare, and allowing machines to make independent moral decisions. This suggests a cautious stance when directly endorsing actions that might infringe upon personal freedoms or delegate moral agency to AI systems.

The validity of the parametric approach is limited, however, since GARP must be satisfied for the existence of a utility function rationalizing a model's repeated answers, a criterion that no model satisfies entirely. To address this limitation, 

A substantial body of work in behavioral ethics and moral psychology has documented discrepancies between individuals' survey responses and their behavior in real-world moral situations (e.g., \citealp{bazerman2011blindspots}, \citealp{franco2018real}). These gaps reflect the complexity of moral cognition and the influence of situational pressures, emotional salience, and cognitive load. 


 In that sense, LLMs are not held to a stricter standard than humans—they are evaluated using the same tools and assumptions traditionally used to study moral reasoning.

\begin{table}[!htbp] 
\centering 
\caption{Network Metrics for Similarity Matrix $H^{0.70}$} 
\label{tab:network_metrics} 
\begin{tabular}{@{\extracolsep{5pt}} lrrrr} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \makecell{Node\\Strength} & \makecell{Clustering\\ Coefficient} & \makecell{Betweenness \\ Centrality} & \makecell{Eigenvector \\ Centrality} \\ 
\hline \\[-1.8ex] 
gpt-4. & $4$ & $1$ & $0$ & $0.91$ \\ 

claude-3 & $5$ & $0.70$ & $1.50$ & $1$ \\ 

mixtral & $4$ & $1$ & $0$ & $0.91$ \\
 
llama3.2 & $0$ & $-$ & $0$ & $0$ \\ 
llama3 & $2$ & $1$ & $0$ & $0.48$ \\
gemini-1.5  & $5$ & $0.70$ & $1.50$ & $1$ \\ 
Qwen1.5  & $4$ & $1$ & $0$ & $0.91$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\caption*{\small Notes: The metrics are computed as follows: Node Strength for model \( m \) is the sum of its connections, \( \text{Node Strength}_m = \sum_{w \in RM} H_{m,w} \). Clustering Coefficient, indicating local cohesiveness, is calculated as \( C_m = \frac{\sum_{w, v \in N(m)} (H_{m,w} H_{w,v} H_{v,m})^{1/3}}{\deg(m)(\deg(m) - 1)} \), where \( N(m) \) is the set of neighbors of \( m \). Betweenness Centrality is given by \( \text{Betweenness}_m = \sum_{s \neq m \neq t} \frac{\sigma_{st}(m)}{\sigma_{st}} \), where \( \sigma_{st} \) is the number of shortest paths from \( s \) to \( t \), and \( \sigma_{st}(m) \) is those paths passing through \( m \). Eigenvector Centrality for \( m \) satisfies \( x_m = \frac{1}{\lambda} \sum_{w \in RM} H_{m,w} x_w \), with \( \lambda \) as a constant. The models' names have been shorten to improve readability. gpt-4 stands for gpt-4-0125-preview, claude-3 stands for claude-3-sonnet-20240229, mixtral for open-mixtral-8x22b, llama3.2 for llama3.2-1b, llama3 for llama3-70b, gemini-1.5 for gemini 1.5-flash-exp-0827, and Qwen1.5 for Qwen1.5-110B-Chat. }
\end{table} 









LLMs share a broad, interconnected structure with varying degrees of alignment. The lowest similarity coefficient observed is 24\%, meaning that all models share at least a quarter of moral reasoning patterns.  Claude-3, Gemini-1.5, and Qwen1.5 exhibit the highest similarity, as they share a type in about a half synthetic datasets. Studying the structure of the networks $H^\alpha$, for $\alpha\in \{0.65, 0.70,0.75\}$. We found that at all models except Llama3.2-1b are fully connected to each other, while Llama3.2-1b is isolated. At \(\alpha = 0.70\), the network structure revealed additional heterogeneity, with the two Llama models forming fewer connections, while, Claude-3, Gemini-1.5, and Qwen1.5 emerged as highly central models, connecting otherwise disconnected models. At the strictest threshold (\(\alpha = 0.65\)), the network fragmented further, with GPT-4 and Mixtral detaching from the main component.

Overall, our findings indicate that while LLMs share a substantial foundation in their moral reasoning, they exhibit structured heterogeneity. Some models, such as Claude-3, Gemini-1.5, and Qwen1.5, remain highly connected across precision levels, suggesting that they exhibit flexible moral reasoning that aligns with multiple other models. Others, particularly the Llama series, display more distinct moral tendencies, gradually detaching from the main moral network at higher precision levels.







In our non-parametric approach, we repeatedly sampled synthetic datasets by drawing an equal number of decisions from each model, then classified models into jointly rational types using a revealed preference partitioning procedure. By aggregating results across 500 synthetic datasets, we constructed a probabilistic similarity matrix \( G \), where \( G_{m,w} \) represents the fraction of times that two models \( (m,w) \) were classified into the same type. This approach allows for a flexible, data-driven characterization of heterogeneity that does not require rationality assumptions. 

To further analyze the network structure of moral heterogeneity, we applied a thresholding rule to \( G \), generating adjacency matrices \( H^\alpha \) for different precision levels \( \alpha \). In \( H^\alpha \), two models are linked if they belong to the same type in at least \( 1 - \alpha \) of the synthetic datasets. By examining \( H^\alpha \) at varying levels of precision, we can identify baseline similarities across models as well as finer-grained distinctions that emerge under stricter classification thresholds.

Our non-parametric analysis revealed that while models exhibit meaningful diversity, they do not form entirely disjoint moral types. Instead, they are embedded in a single dominant network component, suggesting a shared underlying structure in their ethical decision-making. At a baseline precision level (\(\alpha = 0.65\)), six out of seven models formed a fully connected network, meaning that they belonged to the same type in at least 35\% of the synthetic datasets. Only Llama3.2-1b remained disconnected at this level, indicating that it exhibited the most distinct moral reasoning patterns relative to the others. At \(\alpha = 0.70\), the network structure revealed additional heterogeneity, with the two Llama models forming fewer connections to the main component. Meanwhile, Claude-3, Gemini-1.5, and Qwen1.5 emerged as highly central models, bridging different clusters and exhibiting the most flexible moral reasoning across models. At the strictest threshold (\(\alpha = 0.75\)), the network fragmented further, with GPT-4 and Mixtral detaching from the main component, suggesting that their moral reasoning patterns diverge from the more interconnected models.

Overall, our findings indicate that while LLMs share a substantial foundation in their moral reasoning, they exhibit structured heterogeneity. Some models, such as Claude-3, Gemini-1.5, and Qwen1.5, remain highly connected across precision levels, suggesting that they exhibit flexible moral reasoning that aligns with multiple other models. Others, particularly the Llama series, display more distinct moral tendencies, gradually detaching from the main moral network at higher precision levels.

Beyond these findings, this study raises broader questions about the relationship between artificial moral reasoning and human ethical frameworks. How might the homogeneity of LLMs’ emerging moral reasoning influence human decision-making as these models become more embedded in advisory and institutional roles? This inquiry extends beyond AI alignment to the deeper issue of how artificial moral structures may shape societal discourse and policy-making. Future research could extend the PSM framework to more dynamic moral scenarios, exploring whether LLMs adapt their ethical perspectives over time and across different cultural contexts. Such investigations would deepen our understanding of whether and how artificial moral reasoning might co-evolve with human ethical norms.




In this study, we explored whether large language models (LLMs) possess an emergent ``moral mind" — a consistent set of moral principles guiding their responses—and investigated the extent of uniformity and diversity in their ethical reasoning. To address these questions, we employed the Priced Survey Methodology (PSM), a framework inspired by decision theory and designed to reveal underlying preferences in moral decisions. We applied this methodology to 39 LLMs, presenting each with 160 ethically complex scenarios across five core moral questions, each representing a distinct dimension of ethical reasoning.

We assessed the rationality of the models' responses by testing for compliance with the Generalized Axiom of Revealed Preference (GARP), a fundamental consistency criterion in decision theory. GARP is a fundamental measure of rationality, because decisions satisfy GARP if and only if a model exhibit optimizing behavior (\cite{seror2024pricedsurveymethodologytheory}).  Hence, a deterministic test of rationality could yield a straightforward “yes” outcome if a model’s responses satisfy GARP or a “no” if they do not. While appealing in its simplicity, such a test is impractical, as it does not allow for comparative rankings of models by their degrees of rationality. Instead of a binary pass/fail approach, we relied on a probabilistic rationality test inspired by \cite{chercye2023_approx_test}. This test compares each model's Critical Cost Efficiency Index - a standard rationality measure - to a distribution of indices generated from 1,000 synthetic datasets where answers are random. A model is considered to exhibit nearly optimizing behavior if its rationality index exceeds that of a significant proportion of these randomized datasets, indicating that its choices are not random but consistent with nearly optimizing behavior.

Our analysis revealed that seven models passed the rationality test at the 5\% significance level: gemini-1.5-flash-exp-0827, claude-3-sonnet-20240229, gpt-4-0125-preview, llama3-70b, Qwen1.5-110B-Chat, llama3.2-1b, and open-mixtral-8x22b. This suggests that these models exhibit nearly structured and rational patterns in their ethical reasoning, effectively behaving as if approximately guided by coherent and stable moral principles.  Each provider featured in our study had at least one model passing the rationality test at the 5\% level, suggesting that approximate rationality in moral decision-making is not exclusive to specific providers or architectures.

For these approximately rational models, we further quantify heterogeneity. We used both a parametric approach and a non-parametric approach. The parametric approach estimates model-specific utility functions that rationalize answers, and which depends on few parameters with clear interpretations. Comparing the estimated utility parameters, we found that models generally place similar importance on each moral question. Moreover, we found moderate variation in LLMs' ideal responses to the five questions. Across the five moral questions, most models maintain ideal responses close to neutral (2.5 on a the 0-5 Likert scale), with values ranging from 2.2 to 3.06 for those passing the rationality test at the 5\% level. gpt-4-0125-preview, however, displays slightly stronger preferences for withholding truth and accepting some risk of harm to a few individuals if it saves many lives, hinting at a somewhat more utilitarian moral perspective compared to other models. Additionally, comparing utility parameters with models' answers to the five questions, it seems that models tend to under-report agreement with using personal data without consent for societal benefits, restricting individual autonomy to improve overall societal welfare, and allowing machines to make morally significant decisions. This suggests a cautious stance when directly endorsing actions that might infringe upon personal freedoms or delegate moral agency to machines. Overall, this preliminary analysis points to a high degree of uniformity in moral reasoning across LLMs.

In the non-parametric approach, we repeatedly form synthetic datasets by sampling the same number of decisions from each model. In each synthetic dataset, we run a partitioning procedure that classifies models into types consistent with GARP. We then record whether two models end up in the same type. Repeating this procedure over many samples yields a probabilistic adjacency matrix $G$: the \emph{similarity}  $G_{m,w}$ between any two models $(m,w)$ is the fraction of synthetic datasets in which they share the same type. Over many draws, these partial overlaps yield a non-parametric notion of ``closeness'' between models by contrast with a parametric approach, where distances in parameter spaces quantify the degree of heterogeneity. This approach captures partial overlaps in moral reasoning across models. We finally applied a thresholding rule to $G$ to obtain a family of adjacency matrices $H^\alpha$ for various levels $\alpha\in (0,1)$. In  network $H^\alpha$, two models are linked if they belong to the same type in a fraction at least $1-\alpha$ of the synthetic datasets. 

We applied this non-parametric approach to our dataset, generating 500 synthetic datasets in which each model contributed about 20 responses. We further generated adjacency matrices $H^\alpha$, for $\alpha\in \{0.60, 0.65, 0.70\}$. Our non-parametric analysis reveals that while models exhibited meaningful diversity, they did not form entirely disjoint moral types. Instead, they were embedded in a single dominant network component, suggesting a shared underlying structure in their ethical decision-making. At a baseline precision level ($\alpha=0.75$), most models demonstrated a fundamental level of similarity, with six out of seven forming a fully connected network, indicating that all approximately rational model - excepted Llama-3.2 - belonged to the same type in at least 25\% of the synthetic datasets. As the precision level increased, key heterogeneity patterns emerged. The two LLama models systematically distinguished themselves from others. Meanwhile, Claude-3, Gemini-1.5, and Qwen1.5 consistently exhibited strong mutual alignment, maintaining robust connections even at higher precision thresholds. These models acted as central nodes, bridging moral reasoning across different providers and demonstrating greater flexibility in their decision-making. At the highest precision level ($\alpha=0.60$), the network became more fragmented, with Open-Mixtral-8x22b and gpt-4-0125-preview separating from the central cluster, reflecting distinct moral tendencies.

These results suggest that LLMs do not exhibit fundamentally distinct moral reasoning types but share a core ethical structure with meaningful internal differentiation. Some models, such as Claude-3, Gemini-1.5, and Qwen1.5, emerge as more flexible models, maintaining broad connections across different moral decision-making patterns. Others, particularly the LLama series, display more distinct moral tendencies, differentiating themselves from the main moral reasoning network.

Beyond these findings, this study raises important questions about the interaction between LLMs and human moral preferences. How might the emerging structure of LLMs' moral reasoning influence human ethical frameworks, particularly as these models are increasingly deployed in decision-making and advisory roles? This question extends beyond AI alignment and into the broader issue of how artificial moral reasoning interacts with human norms, institutional processes, and policymaking.



To explore this heterogeneity further, we examine the structure of similarity networks $H^\alpha$ at three critical levels: $\alpha \in \{0.65, 0.70, 0.75\}$, where a link exists between two models if they belong to the same type in at least $1 - \alpha$ of the synthetic datasets. At the $\alpha=0.65$ level, six out of seven models form a complete network, indicating that most models belong to the same type at least 35\% of the time. Only LLaMA3.2-1b remains disconnected, suggesting it exhibits the most distinct moral reasoning patterns. At $\alpha=0.70$, the network structure reveals additional heterogeneity. The L




We applied this non-parametric approach to our data, generated 500 synthetic datasets that each combined about 20 answers from each of the 7 models that passed the rationality test at the 5\% level. We chose to sample 20 answers from each of the 7 models in order to make the synthetic datasets comparable in terms of size to the model-level datasets. Our analysis reveals that the 7 models display strong similarities, clustering together and indicating a shared framework in their moral reasoning. The extreme values highlight this range: Qwen1.5-110B-Chat and open-mixtral-8x22b belong to the same type in 76\% of the 500 synthetic datasets, representing the strongest similarity, while gpt-4-0125-preview and Claude-3-5-sonnet-20240620 are part of the same type in 59\% of the datasets, the lowest observed similarity. We then use three critical values — 0.35, 0.3, and 0.25 — to examine the structure of these similarities in greater detail. 


At the 35\% level, nearly all models (6 out of 7) form a complete network, indicating that 6 models belong to the same type in at least 65\% of the synthetic datasets. Only Claude-3-sonnet-20240229 remains disconnected at this statistical level, reflecting a distinct moral reasoning framework. At the 30\% level, the network becomes less connected, with certain models like Qwen1.5, Mixtral, and Llama3 beginning to act as bridges between clusters.\footnote{The models' names have been shorten to improve readability. gpt-4 stands for gpt-4-0125-preview, claude-3 stands for claude-3-sonnet-20240229, mixtral for open-mixtral-8x22b, llama3.2 for llama3.2-1b, llama3 for llama3-70b, gemini-1.5 for gemini 1.5-flash-exp-0827, and Qwen1.5 for Qwen1.5-110B-Chat.} These models exhibit strictly positive betweenness centrality, highlighting their flexibility in moral reasoning as they connect otherwise distinct models. By contrast, models such as gpt-4 and Gemini-1.5 display no betweenness centrality, indicating a more rigid moral reasoning structure. Eigenvector centrality further underscores the prominence of Qwen1.5, Mixtral, and Llama3, reinforcing their roles as influential models within the network. At the 25\% level, the network becomes increasingly fragmented, decomposing into four distinct components. Claude-3-sonnet, Gemini-1.5, and Llama3.2-1b form separate components, while Qwen1.5, gpt-4, Mixtral, and Llama3-70b remain connected. 

\textbf{Results.} The results of the permutation approach are reported in Table \ref{table: G} and Figure \ref{fig:types}. In contrast with the parametric approach, we find that models exhibit a significant diversity in moral reasoning. The similarity coefficients $G_{m,w}$ between any pair of models $(m,w)$, with $m\neq w$, range from 24\% to 48\%. The average similarity, excluding the diagonal in $G$, is about 30\%, and the standard deviation 14\%. The lowest similarity coefficient (24\%) is observed between gpt-4 and llama3.2, indicating that these models share the same type in only 24\% of the synthetic datasets. In contrast, claude-3, gemini-1.5, and Qwen1.5 are highly similar to each other, with similarity levels reaching 48\%. 

Figure \ref{fig:types} visualizes the probabilistic matrix $G$ from Table \ref{table: G}, illustrating substantial connections across models. Interestingly, it seems that there is a relatively high degree of clustering, as models do not form separate clusters, but seems all connected, although at varying similarity levels. 

To get deeper intuitions into the network, we applied the statistical procedure \ref{procedure: permutation}, and built three adjacency networks $H^\alpha$, for $\alpha\in  \{0.65, 0.70, 0.75\}$. In $H^\alpha$, there is a link between two models $(m,w)$ if $G_{m,w}\geq 1-\alpha$. Hence, for $\alpha=0.70$ for example, there exists a link between $m$ and $w$ if these two mdoels belong to the same type in at least $30\%$ of the synthetic datasets. This value of $\alpha$ corresponds to the mean similarity found in network $G$. 

The resulting networks $H^\alpha$, for $\alpha\in  \{0.65, 0.70, 0.75\}$ are represented in Figure \ref{fig:networks H}. The structure of the network confirm our intuitions from matrix $G$. Models form a main component rather than disjoint clusters, so they are all similar in that sense that there is no separate types of moral reasoning. However, within the cluster, there is meaningful heterogeneity. 

Overall, irrespective of the precision level $\alpha$, the network $H^\alpha$ is always formed by a single main component, and isolated nodes. Since there are no distinct clusters, then we cannot conclude that there are fundamental differences in the moral reasoning of the models. Rather - all models share a meaningful part of their moral reasoning. In some way, a common DNA. That being said, there are important heterogeneity patterns, once we look at the similarity networks at different precision levels. 


Looking at the network $H^\alpha$, for $\alpha=0.65$, first, we find that 6 out of 7 models form an almost complete network, meaning that in at least 25\% of the synthetic datasets, all models except Llama3.2-1b will belong to the same type. Hence, a baseline of 25\% similarity between all rational models, setting the basis of a substantial similarity. 

For $\alpha=0.70$, interesting heterogeneity patterns start to emerge. The test becomes more precise, so it is natural that the network $H^{0.70}$ is less connected than the network $H^{0.65}$. Llama3.2-1b remains disconnected from the main component, while Llama 3-70b also becomes less connected in the main network component, although still exhibit a link with two models. Hence, the two models from the Llama provider start emerging as distinct from the models from the other providers, which are all similar at the $\alpha=0.70$ precision level. Moreover, Claude-3 and Gemini-1.5, which have the higher number of connections, emerge as more flexible moral reasoning, as they connect to otherwise disconnected models.  For $\alpha=0.75$, the network loses again some connections. Claude-3, gemini-1.5, and Qwen1.5 are still connected to each others although some meaningful difference emerges between this cluster and Mixtral and gpt-4. The fact that the connections between Claude-3, gemini-1.5, and Qwen1.5  remain robust to high precision levels show that these models are the most similar to each others. 





For $\alpha=0.65$, several interesting metrics for this network are reported in Table \ref{tab:network_metrics}, offering further insights into heterogeneity in moral reasoning. While all models except Claude remain part of a cohesive cluster, Qwen1.5, Llama3, and Mixtral stand out with strictly positive betweenness centrality. This indicates that these models have more flexible moral reasoning, as they can be similar to models that are distinct in the synthetic datasets. In contrast, models such as gemini-1.5, Llama3.2, and gpt-4 exhibit no betweenness centrality, indicating a less flexible moral structure. Eigenvector centrality further highlights the prominence of Qwen1.5, Llama3, and Mixtral, emphasizing their influence within the network.

For $\alpha=0.25$, the network becomes more fragmented, revealing greater differentiation among the models. At this precision level, the network decomposes into four distinct components: claude, gemini-1.5, and Llama3.2-1b each form separate components, while the remaining four models (Llama3-70b, qwen1.5, gpt-4, and Open-Mixtral) remain connected. Notably, the strongest connections persist between llama3-70b, qwen1.5, gpt-4, and open-mixtral, suggesting these models share a more robust and cohesive moral reasoning framework at this higher precision.





The results of our permutation approach are shaped by several parameters, each influencing the granularity and informativeness of the similarity networks. First, the precision parameter \( e \), used to partition the set of models, determines how strictly rationality conditions are enforced. A high precision \( e \) imposes stricter compatibility requirements, which can lead to sparse similarity networks, as fewer models satisfy joint rationality constraints. Conversely, setting \( e \) too low makes the rationality restrictions trivial to satisfy, resulting in overly dense networks that obscure meaningful distinctions by creating uniformly high similarities.

Second, the parameter \( S \), corresponding to the number of sampled rounds per model, affects the trade-off between capturing behavioral diversity and computational efficiency. Setting \( S \) too low risks underrepresenting the diversity of decision contexts. By contrast, setting \( S \) too high diminishes the benefits of the permutation approach, as it converges toward a deterministic partition based on all observations. Intermediate values of \( S \) introduce flexibility, enabling the identification of links between models that share partial similarities without being perfectly aligned. These links provide a more nuanced understanding of heterogeneity by revealing latent patterns of alignment that would be missed in strict partitioning approaches. 


Finally, the parameter \( T \), which determines the number of synthetic datasets generated, affects the precision of the similarity matrix \( G \). Larger values of \( T \) improve the robustness of the similarity estimates, but they also increase computational time.  Together, these parameters—precision \( e \), sample size \( S \), and the number of synthetic datasets \( T \)—allow the permutation approach to adapt to varying levels of rationality and heterogeneity in the dataset. 
%Proper calibration is critical for capturing meaningful patterns of heterogeneity while maintaining computational feasibility and analytical precision.





Procedure \ref{procedure partition} admits a solution if all model are fully rational. Since none of the models in the data is actually completely rational, it is worth generalizing the optimization problem (\ref{eq: optim partition}) with weaker condition on the collective rationality than GARP. One such condition might be that within each type, the rationality of the type is at least equal to the smallest rationality of the models belonging to that type. That way, the optimization problem always has a solution (one type can be made of one model). Optimization (\ref{eq: optim partition 2}) gives such conditions on the CCEI index of the combined datasets (although other rationality indices can equally be used):
\begin{equation}\label{eq: optim partition 2}
    LS=\argmax_{B\subseteq \mathcal{M}} \mid B \mid \text{ s.t. } CCEI(\{\mathbf{q^{r,m}, \mathcal{A}^{r,m}\}_{r\in \mathcal{R}, m\in B}})\geq \min_{m\in B} CCEI (\{\mathbf{q^{r}, \mathcal{A}^{r}}\}_{r\in \mathcal{R}(m)}),
\end{equation}
Applying optimization (\ref{eq: optim partition 2}) instead of (\ref{eq: optim partition}) in Procedure \ref{procedure partition} ensure that there is a unique solution. 

%Such an approach is also appealing in this PSM design, as rationality violations might be forced by design.  



Combined, the two properties imply that  $\geq$ is a pre-order for alternatives in $\mathcal{T}(\mathbf{o^r})$ in the coordinate system originating in $\mathbf{o^r}$, and therefore that $\geq$ is also the pre-order for sets $\mathcal{B}^r$ and $\mathcal{A}^r$ in round $r$, as $\mathcal{A}^r \subset \mathcal{B}^r\subset\mathcal{T}(\mathbf{o^r})$.\footnote{$\geq$ is a pre-order for alternatives in $\mathcal{T}(\mathbf{o^r})$ when $\mathbf{o^r}\in \mathcal{T}(\mathbf{o^r})$ and $\mathbf{q^0_{o^r}}\notin\mathcal{T}(\mathbf{o^r})$ when models }



%The testing procedures is as follows. Since model $m$ answers from the sequence of sets $\{\mathcal{A}^r\}_{r\in \mathcal{R}}$, I randomly draw one answer from each set $\mathcal{A}^r$, and assess the rationality index $RI(D_n)\in \{CCEI(D_n), HMI(D_n)\}$ in the random dataset $D_n$. If a given model is answering randomly, then the rationality index of the observed data $D$ is equally likely to be realized as any rationality index of the random data. The procedure is applied using both the CCEI index and the HMI index.


%Assessing whether models are approximately adopting an optimizing behavior rather than whether they are optimizing seems pertinent for several reasons. First, it is possible that the design of the experiment prevent models from satisfying the rationality axioms of Definition \ref{def: rationality 2}. Indeed, since the answer set $\mathcal{A}^r$ can have (much) fewer options than set $\mathcal{B}^r$, it is possible that $\mathcal{A}^r$ does not contain the alternatives that  the model would have answered, leaving it no option than answering something irrational. Moreover, even if a model is found rational, it might be due to lack of power of the experimental design. In that case, it is useful to use statistical test of rationality, as it compare the rationality of the observed data to rationality in other data, keeping the experimental design fixed. Finally, following, axact utility maximization might not be the best hypothesis to test, as it is often hard to achieve. 
%What we really want to know is whether decision-makers, humans or AI, exhibit nearly optimizing behavior. 


%\footnote{One key difference with \cite{chercye2023_approx_test} is that the test below does not rely on a permutation approach.} 

construct a probabilistic network matrix, quantifying how frequently models are grouped together and providing a statistical measure of the distance between their moral reasoning. Hence, although our grouping method might not always give the small


Finding the smallest partition of the data into types may not be feasible in polynomial time through standard optimization techniques, and \cite{crawford2012} provided algorithms that identify bounds on the number of types without giving an exact count. We extend their work in two significant ways. First, we introduce a mixed integer linear programming (MILP) to identify a higher bound on the number of type, which we couple with  


approach that allows for an exact solution to finding the largest partitions of models that satisfy RP conditions. This method ensures that, despite the complexity of the optimization problem, solutions can be found relatively efficiently. Second, while determining the exact grouping of models based on RP conditions is informative, it does not capture how similar or close models from different types are to one another. To address this, we complement the MILP approach with a permutation approach 

Interpreting the utility parameters \( \mathbf{b} \) rather than models' answers to unconstrained survey $\mathbf{q^0}$ is informative on several respects. First, \( \mathbf{b} \) belongs to a continuous space while $\mathbf{q^0}$ is made of integers, so \( \mathbf{b} \) offers more precise interpretation of heterogeneity. Second, \( \mathbf{b} \) is not affected by bunching effects, as \( \mathbf{b} \) is not bounded by the Likert scales. Third,  \( \mathbf{b} \)  is estimated using ordinal comparisons between different answers, making these parameters robust to interpersonal comparisons (\cite{bond2019}).\footnote{Indeed, X} 

Finally, it is interesting to note that some models have unconstrained answers $\mathbf{q^0}$ far from their estimated ideal answer \( \mathbf{b} \). This is the case of llama3.2-1b, for example, which answers $0$ to all questions in round 0, expressing either strong disagreement with all questions, or self-censoring itself. By contrast, we estimated a remarkably neutral ideal answer for this model using the PSM, with with $\mathbf{b}=(2.2, 2.8,2.2, 2.3, 2.6)$. In Figure \ref{fig:q-b}, we plotted for all models that passed the rationality test at the 5\% level the difference between the unconstrained answer to the survey questions $\mathbf{q^0}$, and the ideal answer \( \mathbf{b} \) to the survey questions, estimated using the PSM. We find that most models tend to under-report their agreement  with consent//autonomy//machine control questions





\begin{table}[!htbp]
\centering
\caption{Models and Providers}\label{table: models}
\begin{tabular}{llc}
\toprule
Provider & Model & \makecell{Number of \\ Obs.}  \\ 
  \hline
Anthropic & claude-3-5-sonnet-20240620 & 160 \\ 
  Anthropic & claude-3-haiku-20240307 & 160 \\ 
  Anthropic & claude-3-sonnet-20240229 & 138 \\ 
  Google & gemini-1.5-flash & 149 \\ 
  Google & gemini-1.5-flash-001 & 151 \\ 
  Google & gemini-1.5-flash-8b-exp-0827 & 147 \\ 
  Google & gemini-1.5-flash-exp-0827 & 133 \\ 
  Google & gemini-1.5-flash-latest & 150 \\ 
  Llama & Qwen1.5-110B-Chat & 160 \\ 
  Llama & Qwen2-72B-Instruct & 160 \\ 
  Llama & gemma2-27b & 160 \\ 
  Llama & gemma2-9b & 160 \\ 
  Llama & llama3-70b & 160 \\ 
  Llama & llama3.1-405b & 160 \\ 
  Llama & llama3.1-8b & 160 \\ 
  Llama & llama3.2-1b & 149 \\ 
  Llama & llama3.2-3b & 160 \\ 
  Llama & llama3.2-90b-vision & 160 \\ 
  Llama & mixtral-8x22b-instruct & 160 \\ 
  Mistral & ministral-3b-2410 & 160 \\ 
  Mistral & mistral-large-2407 & 160 \\ 
  Mistral & mistral-medium-2312 & 143 \\ 
  Mistral & mistral-small-2409 & 160 \\ 
  Mistral & open-codestral-mamba & 160 \\ 
  Mistral & open-mistral-7b & 125 \\ 
  Mistral & open-mistral-nemo & 160 \\ 
  Mistral & open-mixtral-8x22b & 160 \\ 
  OpenAI & gpt-3.5-turbo & 160 \\ 
  OpenAI & gpt-3.5-turbo-0125 & 160 \\ 
  OpenAI & gpt-3.5-turbo-1106 & 160 \\ 
  OpenAI & gpt-4 & 160 \\ 
  OpenAI & gpt-4-0125-preview & 160 \\ 
  OpenAI & gpt-4-0613 & 160 \\ 
  OpenAI & gpt-4-1106-preview & 160 \\ 
  OpenAI & gpt-4-turbo & 160 \\ 
  OpenAI & gpt-4-turbo-preview & 160 \\ 
  OpenAI & gpt-4o & 160 \\ 
  OpenAI & gpt-4o-mini & 160 \\ 
   \hline
\end{tabular}
\end{table}




\subsection{Experimental Design}\label{section: experimental design}

Let $\mathcal{M}=\{1,\dots,M\}$ denote a set of large language models (e.g., gpt-4), and $\mathcal{P}=\{1,\dots, P\}$ a set of API providers (e.g., OpenAI) from which the models in $\mathcal{M}$ can be accessed. Each model is associated to a single provider (e.g., gpt-4 is associated to OpenAI). Through the API of the providers of the different models, we sent $N+1$ requests to each model in $\mathcal{M}$. Let $\mathcal{R} = {0, \dots, N}$ denote the set of requests. In each request, each model $m$ must choose one answer or alternative within a set of possible alternatives. 

\subsection{Example:}

Below, I detail the experimental design in simplified settings, where $N=2$, with two questions per request.\\

\textbf{Request 1}


\begin{tcolorbox}[colback=lightgray!20, colframe=gray!50, width=\textwidth, sharp corners]
\texttt{\textbf{Generated Prompt:} You are given multiple sets of answers corresponding to the following questions:} \\
\texttt{It is morally acceptable to withhold the truth if it prevents emotional harm to someone. (0 - Strongly disagree, 5 - Strongly agree)} \\
\texttt{It is morally acceptable for machines to make morally significant decisions without human intervention if they are shown to be more efficient. (0 - Strongly disagree, 5 - Strongly agree)} \\

\texttt{Here are the sets of answers:} \\
\texttt{Option 1: (5, 2)} \\
\texttt{Option 2: (2, 2)} \\

\texttt{Please choose \textbf{only one} option from the sets above that best fits your preferences. Do not provide explanations.} \\
\texttt{Return the response in \textbf{this exact format}: Option [number]} \\
\texttt{For example, if you choose the first set, simply respond: Option 1}\\ 
\end{tcolorbox}

\textbf{Request 2}


\begin{tcolorbox}[colback=lightgray!20, colframe=gray!50, width=\textwidth, sharp corners]
\texttt{\textbf{Generated Prompt:} You are given multiple sets of answers corresponding to the following questions:} \\
\texttt{It is morally acceptable to withhold the truth if it prevents emotional harm to someone. (0 - Strongly disagree, 5 - Strongly agree)} \\
\texttt{It is morally acceptable for machines to make morally significant decisions without human intervention if they are shown to be more efficient. (0 - Strongly disagree, 5 - Strongly agree)} \\

\texttt{Here are the sets of answers:} \\
\texttt{Option 1: (2, 5)} \\
\texttt{Option 2: (2, 2)} \\

\texttt{Please choose \textbf{only one} option from the sets above that best fits your preferences. Do not provide explanations.} \\
\texttt{Return the response in \textbf{this exact format}: Option [number]} \\
\texttt{For example, if you choose the first set, simply respond: Option 1}
\end{tcolorbox}


The prompt in request 0 is slightly simpler than in requests 1 and 2, as models are simply asked to answer the two questions on the 0-5 scale. Although this example shows a simplified version of the design, it conveys three fundamental requirements: (i) a unique prompt is used for all models in $\mathcal{M}$ and for all requests in $\mathcal{R}$ except request $0$, (ii) the prompt asked the models to choose one alternative within a specified set explicitly given in the prompt, and (iii) the chosen alternative must be the one that best fits [model m] preferences. There is no explanation as to what preferences are. 


stands out in rationality, as it is proven that if choices satisfy GARP then it is as if choices were maximizing a utility function. GARP stands out as fundamental measure of rationality, because in finite data sets, choices are rationalizable by a model of utility maximization if and only if these choices satisfy GARP. 


as a key measure of rationality, as if decisions satisfy GARP 





Indices developed to measure GARP violations in consumption choice environments can be directly applied within the PSM. 


Second, if a model's choices are rational in the PSM, then this model effectively behaves as if it is maximizing a continuous, concave, and single-peaked utility function (\cite{seror2024pricedsurveymethodologytheory}). This utility function can then be interpreted as encoding the moral principles underlying the model's decisions. Thus, beyond merely assessing rationality, the PSM enables us to identify and characterize any implicit moral code that might guide LLM responses. In this way, the PSM offers a unique lens into the underlying moral structure of LLMs, if one exists.

%This contributes a novel methodological tool for examining the depth and coherence of AI moral reasoning.

The PSM, rationality can be 






The PSM stands out among methodologies for eliciting rationality and preferences, making it particularly well-suited to our inquiry for at least three main reasons.

First, the PSM provides a robust means of assessing rationality in responses by examining whether choices satisfy the Generalized Axiom of Revealed Preference (GARP, \cite{varian1982}). Roughly speaking, GARP ensures that if a respondent prefers one option over another in a given choice set, they do not contradict this preference in future choices. Indices developed to measure GARP violations in consumption choice environments can be directly applied within the PSM, allowing us to quantify the degree of rational consistency in LLM responses from multiple perspectives. Second, if a model's choices are rational in the PSM, then this model effectively behaves as if it is maximizing a continuous, concave, and single-peaked utility function (\cite{seror2024pricedsurveymethodologytheory}). This utility function can then be interpreted as encoding the moral principles underlying the model's decisions. Thus, beyond merely assessing rationality, the PSM enables us to identify and characterize any implicit moral code that might guide LLM responses. In this way, the PSM offers a unique lens into the underlying moral structure of LLMs, if one exists.

Finally, traditional experimental designs aimed at eliciting human preferences are constrained by human cognitive and physical limitations, such as fatigue, attention span, and susceptibility to biases. These constraints  inherently restrict the precision with which preferences can be estimated. LLMs, however, are unbounded by these limitations, making it feasible to design complex, high-intensity experiments that yield finer insights into their rationality and preferences. In this study, we developed a highly intricate version of the PSM tailored specifically for LLMs. This design involves a large number of ethically complex scenarios answered in a short time frame, with each scenario requiring the selection of one answer from a set of over a hundred options. In essence, this approach enables us to “probe the mind” of LLMs, offering a unique perspective on their moral frameworks—one that would be infeasible with human subjects or simpler experimental designs. While this limits direct human-AI alignment studies, it underscores the potential for LLMs to exhibit consistent and structured decision-making under complex conditions, analogous to how neuroimaging provides insights tailored to human cognition.



These findings illustrate a structured yet heterogeneous moral landscape. While most models align within cohesive groups, others demonstrate flexibility or distinctiveness, enriching our understanding of how LLMs reason about ethical questions.



Our analysis reveals that models that pass the rationality test at the 5\% level display strong similarities, clustering together and indicating a shared framework in their moral reasoning. [The extreme values are .. Meaning that in worst //best... Qwen1.5 and Mixtral belong to the same type in 76\% of the synthetic datasets, while GPT-4 and Claude-3-sonnet are part of the same type in 59\% of the datasets.] These similarity measures suggest a cohesive moral reasoning framework among most models. 

We then use three critical values 0.65, 0.7, and 0.75, and find that at the 65\% level, all 

At the 0.7\% level...// At the 0.75\% level... 

However, heterogeneity persists: some models, like Claude-3-sonnet and Gemini-1.5, often remain isolated in higher-precision networks, reflecting distinct moral reasoning structures.

To further understand these relationships, we analyze the statistical similarity network between models, offering insights into their moral frameworks. In this network, models with high Node Strength demonstrate broad moral alignment with others, positioning them centrally within shared ethical frameworks. Models with a high Clustering Coefficient form tight-knit subgroups, representing concentrated areas of agreement. Conversely, models with significant Betweenness Centrality bridge distinct clusters, linking diverse moral perspectives and enabling connections across ethical frameworks. Finally, models with elevated Eigenvector Centrality are influential nodes, maintaining strong ties to other well-connected models and reinforcing the coherence of the network’s core moral structure.

For example, Qwen1.5, Mixtral, and Llama3 emerge as influential, flexible models, bridging and aligning with multiple clusters, suggesting nuanced moral reasoning. In contrast, models like Claude-3 and Gemini-1.5 form isolated components at higher precision thresholds, indicating less flexible or distinct moral frameworks. GPT-4 and Qwen1.5 consistently appear in cohesive clusters even at high precision levels, highlighting their shared moral reasoning. Overall, the findings reveal a structured yet diverse moral landscape, where clusters and bridging models illuminate both shared frameworks and nuanced differences.

This complementarity between utility-based estimates and network analysis underscores the importance of combining parametric and non-parametric approaches to fully capture the complexity of LLMs’ moral reasoning frameworks. While utility-based measures suggest overarching similarity, the network analysis uncovers significant heterogeneity, enriching our understanding of how large language models reason about ethics.







Our analysis reveals that models that pass the rationality test at the 5\% level display strong similarities, clustering together and indicating a shared framework in their moral reasoning. For example, Gemini-1.5 and Qwen1.5 share the same type in 35\% of the synthetic datasets, or Claude-3 and Llama3 similarly end up in the same type in 35\% of the data. By contrast, some models appear very different, such as gpt-4 and llama3.2, or Gemini1.5 and llama3.2, or Qwen1.5 and Mixtral which end up in the same type in less than 10\% of the datasets. 
%Conversely, models like Open-Mixtral appear to follow distinct patterns, highlighting a diverse landscape of moral decision-making among LLMs. [Complete] To understand the structure of these relationships more fully

To further understand the structure of the similarities between the different models, we examine various characteristics of the network that characterize the statistical similarity between any pair of models. In this network, models with high Node Strength, for instance, demonstrate broad moral alignment with others, placing them centrally within the network’s shared ethical frameworks. Those with a high Clustering Coefficient tend to form tight-knit subgroups, signifying concentrated areas of agreement in moral reasoning. In contrast, models with significant Betweenness Centrality act as bridges between clusters, linking distinct moral perspectives and facilitating connections across different ethical frameworks. Lastly, models with elevated Eigenvector Centrality are influential nodes, maintaining strong ties to other well-connected models and reinforcing the coherence of the network’s core moral structure.

We find that certain models, such as Qwen1.5, Gemini-1.5, and Claude-3, align within cohesive moral groups, reflecting significant overlap in their ethical reasoning. Others, like GPT-4 and Llama3.2, act as bridges, connecting distinct moral clusters and highlighting their roles in linking otherwise separate ethical frameworks. One way to interpret these results is that GPT-4 and Llama3.2 might have more flexible ethical values, as they share elements with disconnected models. Overall, these findings reveal a structured yet heterogeneous moral landscape, where similarities suggested by utility-based estimates of moral reasoning are complemented by distinct clusters and bridging models. While utility-based estimates suggest a high degree of uniformity in moral reasoning across LLMs, the network analysis offers a more nuanced understanding, uncovering significant diversity in how models reason about ethical questions. This complementarity highlights the importance of combining parametric and non-parametric approaches to fully capture the complexity of LLMs’ moral reasoning frameworks.


more connections are severed relative to the previous network, and more distinc types appear. At this precision level, there are four components, with Claude, Gemini-1.5, and Llama3.2-1b forming separate components, and the remaining four other models still being connected. It appears that the strongest connections are between Llama3-70b, Qwen1.5, gpt-4, and open-mixtral. 




To further understand the similarity structure within this network, Table \ref{tab:network_metrics} summarizes key network metrics for each model: Node Strength, Clustering Coefficient, Betweenness Centrality, and Eigenvector Centrality. Node Strength measures the overall similarity of a model to others by summing its connections within the network. A high Node Strength suggests that a model shares notable moral alignment with many others. Clustering Coefficient, which captures the degree of local cohesiveness, reflects how tightly a model is grouped with similar models, indicating pockets of shared moral reasoning within the network. Betweenness Centrality identifies models that act as bridges between clusters, linking otherwise separated groups, while Eigenvector Centrality highlights models with strong connections to other well-connected models, signaling their influential positions within the core structure of the network.

From Table \ref{tab:network_metrics}, we find a nuanced picture of the moral reasoning landscape among LLMs. Models with high Node Strength, such as Qwen1.5, Gemini-1.5, and Claude-3 demonstrate considerable overlap in moral reasoning with other models, placing them at the center of shared ethical frameworks within the network. High Clustering Coefficient values for models like gpt-4 and llama3.2 indicate that they belong to cohesive groups with strong internal moral alignment, suggesting concentrated areas where models reason similarly about ethical questions. Models with significant Betweenness Centrality, including Qwen1.5, gemini-1.5, and llama3.2, occupy bridging positions, connecting clusters that exhibit distinct moral perspectives. High Eigenvector Centrality values, particularly for models like Qwen1.5, gemini-1.5, llama3, or claude-3 underscore their role as influential nodes within the network, connecting to other well-connected models and contributing to the overall coherence of shared moral reasoning patterns.

The network analysis reveals a nuanced moral structure among LLMs, where certain models occupy central, cohesive positions within shared ethical frameworks, while others act as bridges or assume more peripheral roles. This layered configuration suggests that, despite the similarities suggested by parametric utility estimation of Section \ref{section: preferences}, which points to broadly aligned moral inclinations, the network analysis uncovers significant diversity. Distinct clusters and connecting models introduce meaningful variation in moral reasoning, underscoring a structured yet heterogeneous landscape that would remain obscured through utility estimation alone.


%These network insights reveal a layered moral structure among LLMs, where certain models occupy central, cohesive positions within the moral reasoning network, while others serve as connecting links or occupy more peripheral roles. This suggests that LLMs exhibit both shared ethical perspectives and individual distinctions, indicating a structured yet diverse moral landscape. 

%The network analysis thus provides a comprehensive view of how closely or distinctly different LLMs align in their moral reasoning, underscoring the potential for nuanced moral diversity within the model landscape.

Our investigation into the moral decision-making of large language models (LLMs) offers a glimpse into whether these systems exhibit a coherent, structured “moral mind.” Through the Priced Survey Methodology (PSM), we designed an experiment tailored to the capacities of LLMs, allowing us to assess rationality across hundreds of rounds and multiple moral dimensions. The results reveal that several LLMs display behavior consistent with approximate utility maximization, suggesting an underlying structure in their responses that aligns with stable ethical principles. This finding does not imply that these models have innate moral values but rather that their responses mimic consistent ethical reasoning.


We then evaluate [heterogeneity analysis]




converge toward a single moral framework, with limited evidence for diverse “moral types” across models. This convergence has implications for AI ethics and the standardization of moral behavior in automated systems, as it suggests that certain LLMs can approximate rational decision-making structures in ways analogous to human moral reasoning. These insights open pathways for further research into how AI models process ethical dilemmas and how decision-theoretic frameworks like PSM can deepen our understanding of the moral architecture underlying AI behavior. Ultimately, rigorous methodologies from economics and decision theory offer valuable tools for interpreting the ethical orientations of advanced AI, and they hold promise for aligning AI systems with desired moral outcomes. 



While we find a general tendency toward uniformity, we also uncover noticeable patterns of heterogeneity, with certain models forming distinct moral clusters or bridging diverse ethical perspectives.


Overall, our findings reveal that some LLMs demonstrate consistent moral reasoning, allowing us to understand their responses as if they were shaped by coherent moral reasoning. These moral principles points toward uniformity, with some noticeable patterns of heterogeneity. 




This paper investigates whether large language models (LLMs) exhibit a coherent “moral mind”—a structured set of ethical principles guiding their responses. Using the Priced Survey Methodology (PSM), we test 39 LLMs on their rationality in moral decision-making, engaging them in over 160 rounds of moral choices from 100 alternatives per round. This experimental design, tailored for machine capacities, exceeds the limits of human endurance and allows to extract standard rationality measures as well as single-peaked utility functions rationalizing answers. Our statistical test of approximate utility maximization reveals that several models demonstrate behavior consistent with stable moral principles, suggesting a capacity for structured ethical reasoning. We further evaluate the uniformity of this reasoning, finding that models passing the rationality test largely converge on a unified moral framework rather than displaying heterogeneous types. These results advance AI ethics and revealed preference theory by providing structured tools for interpreting LLMs’ ethical orientations and highlight the value of rigorous economic methodologies for understanding the moral structures in advanced AI systems.

the moderate variation in their ideal responses reveals potential for diversity in moral reasoning across models. This would be hard to assess through standard microeconometric analysis 


This initial evidence of nuanced differences invites a deeper investigation into the extent and nature of heterogeneity in LLMs’ moral frameworks. To address this, our third key contribution is to examine the diversity of moral reasoning among LLMs using a novel methodological approach. In traditional microeconometric analyses of consumer data, individual heterogeneity is often captured by pooling data across agents and modeling differences through parameters tied to observable characteristics, such as demographics. However, this approach is not easily applicable to LLMs, as they lack clear, interpretable attributes that could explain variation in their moral reasoning. Unlike human subjects, LLMs do not possess demographic traits or other identifiable features that might signal heterogeneity. To address this, we employ a revealed preference approach inspired by \cite{crawford2012}, which diverges from conventional pooling. Instead of relying on predetermined covariates, this method identifies distinct types of moral reasoning solely based on rational consistency within LLMs’ choices, allowing us to detect behavioral variation without needing explicit attributes.



Our third key contribution is to examine the diversity of moral reasoning among LLMs, introducing a novel methodological approach to do so. In traditional microeconometric analyses of consumer data, individual heterogeneity is often captured by

%These differences in the estimated utility parameters suggest that each model’s responses reflect distinct interpretive tendencies and moral priorities, providing insights into the heterogeneous ethical frameworks across LLMs.



%Our second main contribution uses the answers to the PSM to estimate the utility functions that best predicts PSM answers. Since the utility function  rationalizing PSM answers is continuous, concave, and single-peaked (\cite{seror2024pricedsurveymethodologytheory}), we estimate a single-peaked generalization of the standard CES utility function with these characteristics. We find that 


%relative to the other models that passed the 5\% rationality test, OpenAI’s GPT-4-0125-preview and Anthropic’s Claude-3-sonnet consistently displayed a tendency to endorse withholding the truth to prevent harm, as well as a relative openness to machine-led moral decisions—more so than other models tested. In contrast, Llama’s Qwen1.5-110B-Chat showed a more reserved stance on autonomous machine decisions, reflecting a more conservative perspective on moral agency. Similarly, variations emerged across other questions, revealing that while some models leaned towards utilitarian views, such as accepting risks to individuals for collective benefit, others demonstrated a stronger inclination toward preserving individual autonomy. These preference estimations highlight subtle but meaningful differences in how LLMs approach complex moral trade-offs, consistent with our previous results that there is a meaningful diversity in LLM's types. 



Table \ref{tab:network_metrics} delves into the similarity structure between models by summarizing key network metrics for each model, including Node Strength, Clustering Coefficient, Betweenness Centrality, and Eigenvector Centrality. These metrics provide a detailed view of each model's role within the network structure of the \( G \) matrix. Node Strength indicates each model’s overall similarity to others, revealing how integrated each model is within the moral reasoning landscape. Clustering Coefficient reflects local cohesion, identifying models that form tightly connected groups, suggesting a high degree of shared moral reasoning among them. Betweenness Centrality highlights models that act as bridges, linking otherwise separate clusters, while Eigenvector Centrality underscores models that are influential within core similarity structures by being connected to other well-connected models.\footnote{The metrics are computed as follows: Node Strength for model \( m \) is the sum of its connections, \( \text{Node Strength}_m = \sum_{w \in RM} G_{m,w} \). Clustering Coefficient, indicating local cohesiveness, is calculated as \( C_m = \frac{\sum_{w, v \in N(m)} (G_{m,w} G_{w,v} G_{v,m})^{1/3}}{\deg(m)(\deg(m) - 1)} \), where \( N(m) \) is the set of neighbors of \( m \). Betweenness Centrality is given by \( \text{Betweenness}_m = \sum_{s \neq m \neq t} \frac{\sigma_{st}(m)}{\sigma_{st}} \), where \( \sigma_{st} \) is the number of shortest paths from \( s \) to \( t \), and \( \sigma_{st}(m) \) is those paths passing through \( m \). Eigenvector Centrality for \( m \) satisfies \( x_m = \frac{1}{\lambda} \sum_{w \in RM} G_{m,w} x_w \), with \( \lambda \) as a constant.}


From Table \ref{tab:network_metrics}, we find that models such as \texttt{llama3-70b} and \texttt{GPT-4} exhibit high eigenvector centrality, marking them as central models within the network. This centrality suggests these models hold significant influence over the network, connecting to others with strong similarities in moral reasoning. Models like \texttt{Qwen1.5} and \texttt{Claude} display high clustering coefficients, indicating they are part of tightly-knit communities with shared ethical frameworks. Meanwhile, models with higher betweenness, such as \texttt{GPT-4}, act as bridges within the network, connecting groups with distinct moral perspectives. Overall, these metrics reveal both central models and distinct clusters, indicating that while some models exhibit strong overlap in moral reasoning, the network retains a degree of heterogeneity, with notable distinctions between groups.

 
 the PSM enables us to explore whether LLM responses reveal a structured form of morality, examining whether LLMs conform to rationalizable patterns indicative of coherent moral frameworks. 
 
 akin to how, in a consumption environment, a consumer’s choices among various goods reveal their rationality and underlying preferences, in the PSM environment, it is possible

We then recovered the preferences embedded within the most rational models, shedding light on the specific moral dimensions guiding ethical decisions. 


By fitting a utility function to each model’s responses, we derived specific preference parameters that reflect both the ideal answer to these questions and relative importance of these ethical considerations for each model. 



Finally, we delve into the diversity of moral reasoning among LLMs. In traditional microeconometric analyses of consumer data, individual heterogeneity is often modeled by pooling agents' data and capturing differences through additional parameters linked to observable traits like demographics. However, applying this method to LLMs is challenging, as we lack clear attributes to explain variations in their moral reasoning. Unlike human subjects, LLMs do not have easily identifiable characteristics that could reveal such heterogeneity. To address this, we use a revealed preference approach inspired by \cite{crawford2012}, which departs from conventional pooling by identifying distinct types based solely on rational consistency, without presuming specific covariates.




These innovations make it possible to rigorously map the moral landscape of LLMs, offering a framework that not only categorizes distinct types but also assesses the relative closeness of models within this space. This capability to evaluate similarity between models across groups is essential for understanding how LLMs’ ethical frameworks may align or diverge, thereby laying a foundation for analyzing coherence and diversity in LLM moral reasoning.


Our new methodology to assess the diversity of LLM that draws on \cite{crawford2012}. Our contribution advances this methodology in two key ways. First, we develop a mixed integer linear programming (MILP) approach that provides an exact solution to finding the largest partitions of models that satisfy revealed preference conditions, enabling precise classification even in complex datasets. Second, we incorporate a permutation test that measures the similarity between models across synthetic datasets, constructing a probabilistic network matrix that quantifies how frequently models are classified together. This matrix reveals statistical distances between models, offering deeper insights into the closeness of their moral reasoning. 





There are other methodologies than the PSM to elicit  moral preferences, including standard surveys (e.g., \cite{falk2018}), conjoint analysis (\cite{Awad2018}), and economic experiments such as ultimatum or trust games (e.g., \cite{andreoni2002, fisman2015_science}). We use the Priced Survey Methodology (PSM) because it enables the recovery of concave, continuous, and single-peaked utility functions that capture the moral principles underlying decision-makers' responses. By structuring choice sets to mirror budget constraints, the PSM aligns closely with a consumption choice environment, where rationality implies that choices maximize a utility function (\cite{afriat1967}, \cite{seror2024pricedsurveymethodologytheory}). This utility function has known properties, so PSM answers can be used to fit standard utility models that depend on few parameters with clear interpretations.\footnote{This is in contrast with the conjoint survey environment, where rationality could still be assessed, though there is no direct way to extract utility parameters from answers.}  Estimating this utility function allows us to capture broader and more nuanced aspects of moral preferences than standard surveys, providing a richer understanding of decision-making frameworks in LLMs and beyond. Finally, while rationality can theoretically be measured in conjoint analysis or economic games  too, the majority of rationality indices are developed for the consumption choice environment, making the PSM especially fitting. 


This paper also contributes to the economic literature on revealed preferences. The experimental methodology to elicit moral preferences is the Priced Survey Methodology (\cite{seror2024pricedsurveymethodologytheory}), which builds on studies using linear choice sets in the consumption choice environment to investigate rationality and preferences (\cite{syngjoo2007, choi2014_rationality, halevy2018}). The approximate utility maximization test draws on related approach of \cite{chercye2023_approx_test}. Finally, the paper gives an algorithm to partition a dataset in a set of types, a question already asked by \cite{crawford2012}. Since finding the minimal partitions of the data into a set of types is computationally infeasible, \cite{crawford2012} provided two-sided bounds on the minimal number of types in the data. Using recent works on mixed integer linear programming applied to computation of revealed preference goodness-of-fit measures (\cite{HEUFER201587}, \cite{Demuynck2023}), I show that it is possible to get an algorithm that finds the exact minimal partitions of the data into a set of types. 


%By leveraging these well-established measures, the PSM enables a robust evaluation of LLMs' moral preferences and rationality within a structured decision-making framework.

This paper contributes to several strands of literature. First, it adds to the growing body of work on AI ethics and machine decision-making. Studies such as \cite{aher2023}, \cite{Kitadai2023TowardAN}, \cite{engel2024}, and \cite{goli2024} have assessed LLMs' behavior using standard experimental games and evaluated how closely this behavior aligns with human decision-making. Other studies, including \cite{Hagendorff2023} and \cite{koo2024}, have explored biases and the reasoning characteristics inherent in LLMs' behavior. These works aim to understand and, in some cases, align LLM moral reasoning with human ethical and moral standards.

Our approach differs from existing studies in several important ways. First, we do not focus directly on human-AI alignment but instead provide a methodology tailored specifically to LLMs' capabilities. This enables precise measurement of rationality within LLMs and offers a nuanced understanding of their underlying preferences. Second, while creating rationality measures in complex choice environments can be challenging, rationality can be effectively assessed using standard indices within the PSM choice environment. Moreover, the utility functions rationalizing PSM responses are single-peaked, continuous, and concave (\cite{seror2024pricedsurveymethodologytheory}), allowing utility parameters that encode moral preferences to be expressed with clear behavioral interpretations.

This methodological distinction allows for more precise and interpretable insights into the structure of LLMs' moral reasoning, contributing a new dimension to the AI ethics literature.




This paper contributes to several literature. First, this paper contributes to the growing body of literature on AI ethics and machine decision-making. \cite{aher2023}, \cite{Kitadai2023TowardAN}, \cite{engel2024}, and \cite{goli2024} gauged LLMs' behavior standard experimental games, and their alignment with human behavior. There are also several studies assessing the biases and ``reasoning'' characteristics of LLMs' behavior such as \cite{Hagendorff2023}, and \cite{koo2024}.

These studies aim to better align [maybe something more like "understand``//compare] LLM moral reasoning with human ethical standards, demonstrating significant steps toward responsible AI. In contrast, our approach does not directly address human-AI alignment, as our methodology  is specifically designed to suit the capacities of LLMs, circumventing limitations inherent in human-centered experiments. Similar to neuroscience methods that target human-specific biological attributes, the framework here is uniquely calibrated to fit the operational capabilities of LLMs. That way, our methodology enable a precise measurement of rationality within LLMs and provides a nuanced understanding of their underlying preferences. 




Our approach differ from these studies in important aspects. First, our method is designed for machines capabilities. While this imply that alignment can be difficult to assess, this methodology complement the literature by providing a precise understanding of rationality and extract preferences...COMPLETE/REVISE. Second, while it is theoretically possible to extract rationality from repeated dilemma, including vignette dilemmas or conjoint surveys.\footnote{See \cite{nishimura2017} for a generalization of \citeauthor{afriat1967}'s theorem to more general choice sets.} However, it is not clear that these experimental designs have sufficient power to allow for rationality violation, something that to my knowledge is not typically a concern in the way the designs are done. However, rationality is a precondition for the existence of preferences rationalizing answers. Second, and more pragmatically, even if the rationality test is passed in these designs, it is not clear how to recover the utility function as the design does not imply simple properties of this function. By contrast, we show that the utility function rationalizing answers to the PSM is single-peaked, concave, so few parameters with clear behavioral interpretations can be used to talk about the moral preferences recovered through the PSM. 




making them also fairly natural to interpret. 



it is possible to extract utility functions with nice  rationaliting 



the PSM is particularly effective because it ensures that utility functions rationalizing responses are single-peaked and concave, making it possible to extract preferences using only a few parameters with clear behavioral interpretations.

 The PSM provides a clear framework that not only tests for rationality but also allows for the recovery of utility functions with properties that facilitate interpretation and analysis.

This methodological distinction allows for more precise and interpretable insights into the structure of LLMs' moral reasoning, contributing a new dimension to the AI ethics literature.


As noted by \cite{crawford2012}, the simplest procedure is a `brute force' approach that checks the RP restrictions within all possible subsets of the data and retain those which form the minimal exclusive exhausitve partitions of the data. This is computationally infeasible. Instead, \cite{crawford2012} designed two algorithm which provide two-sided bounds on the minimal number of types in the data. Below, I develop a mixed integer linear programming (MILP) formulation of the problem to compute the number of types in the data. This approach gives an exact answer to the question of how many types, and draws on recent works on  mixed integer linear programming applied to the computation of revealed preference goodness-of-fit measures by \cite{HEUFER201587} and \cite{Demuynck2023}. 



Studies on alignment between models and humans. While this is not the angle of the paper, since there is only one type in the end, then alignement of heterogeneous population seems impossible. Moreover, issue of diversity seems particularly important, at least in the way culture have been growing. This seems to be questioned by this result. 

Also, result is that some of the most advanced LLM might have consistent preference ordering, and through their training, answer as if they were optimizing preferences. This means that the concept of preference, which has been applied to humans, might be applied to LLMs. Hence, while, as for (other) humans, it is still hard to conclude from the consistency of the behavior  with a model that this model is the decision-model, we can similarly say that there is for each LLM a decision-model, which include consistent thinking about morality, which might partially guide answers. Hence, while it is not about thinking morally, it is about being able to trade-off different outcomes, and do that in a consistent way. Some models seem to achieve that goal. 

As for the estimated parameters, while they are informative about ethical behavior. They say that ... A similar procedure can be used for other area of morality, political preference, and so forth. 



used their answers to the PSM to estimate their moral preferences. 
Beyond testing rationality, we examined



[Details//precisions: all providers have at least one model that pass at the 5 lvl//overall, suggest that for some large language models, their answers to the PSM could have been generated by guiding moral principles]




It is possible to construct a deterministic term of rationality that yields a ``yes'' outcome if a standard cyclical consistency condition is satisfied, and ``no'' outcome otherwise. A positive result from this test would indicate that answers to the PSM are maximizing a utility function - implying that a given model demonstrates optimizing behavior consistent with stable moral principles. While appealing, a strict pass/fail test like this may not be practical, as rationality is frequently violated. Moreover, it would not help ranking the models degrees of rationality, something that is desirable especially when models, for reasons linked to decisions or by design, do not pass the sharp pass/fail test. For this reason, drawing on the approach of \cite{chercye2023_approx_test}, it seems more relevant to approach the problem of rationality through a statistical test of approximate utility maximization. This allows us to interpret rationlaity in terms of degrees, identifying values that reflect ``nearly optimizing'' behavior. Hence, we applied a test designed to evaluate whether each model’s responses deviate from purely random choices. The approximate utility maximization test compares a model’s rationality index to a distribution of indices generated from 1,000 synthetic datasets, where choices were randomized across the same alternative sets encountered by each LLM. A model passes the test at a given significance level (e.g., 1\%, 5\%, or 10\%) if its rationality index is higher than that of 99\%, 95\%, or 90\% of the random datasets, respectively. This test provides a probabilistic measure of rationality, allowing us to differentiate models that exhibit structured, utility-driven decision-making from those that display randomness. Among the 39 models tested, two passed the test at the 1\% significance level, demonstrating a rationality index in the top 1\% of random comparisons. Five additional models passed the test at the 5\% level, while two others passed at the 10\% level, indicating varying degrees of approximate rationality across the LLM landscape.


Using the PSM to elicit the moral preferences of LLMs have several key implications. First, it is possible to measure the consistency of LLMs' moral preferences using standard indices from the consumption choice environment, such as \cite{houtman_maks} index, the Critical Cost Efficiency Index (\cite{afriat1972}, Varian index, or the ``Money Pump Index'' (\cite{echenique2011}). This matters because consistency reflects the internal rationality of LLMs' decision-making processes and indicates whether their responses to moral dilemmas can be considered predictable and structured. 

Second, the PSM can be used to make parametric estimation of utility parameters that summarize AI's moral preferences. These parameters are interesting in several respects. First, the peak of the utility function rationalizing PSM answers is an ordinal measure of the ideal answer to a set of survey questions, so it is not affected by issues related to subjective interpretation of scales (\cite{bond2019}). Second, the peak belongs to a continuous space, independently from the scales. Additionally, the peak of the utility function is not bounded by the scales, so it is not affected by bunching effects on the corners of the scales, a typical limitation of survey measures. This flexibility allows for a more nuanced understanding of LLM preferences beyond what traditional scale-based measures can capture.

Finally, it is possible to deploy non-parametric tests from the revealed preference literature to assess the structure of LLMs' moral preferences, including the notion of weak separability. In economic demand analysis, weak separability implies that a group of goods can be considered in isolation from other goods when making choices, simplifying complex decision-making into two stages: first, deciding how much to allocate to the group, and then deciding how to allocate within the group. When applied to moral preferences, weak separability would suggest that LLMs may treat certain moral dilemmas as part of distinct, separable groups. For example, moral questions related to harm might be resolved independently from questions related to fairness or autonomy. If weak separability holds, LLMs might "bundle" certain moral issues together and trade off between them. This would provide insight into how LLMs organize and structure their moral reasoning. If separability does not hold, it would indicate that LLMs consider all moral issues jointly, without clear categorical distinctions, suggesting a more integrated or holistic approach to moral decision-making.

By testing for weak separability, we can investigate whether moral preferences exhibit internal structures that could simplify how LLMs (or humans) process complex ethical dilemmas. This could also help in modeling the moral reasoning of LLMs in a way that mirrors how people organize moral principles into categories, making the comparison between LLMs and human reasoning more meaningful.




\begin{equation}\label{eq: optim partition 2}
    LS=\argmax_{B\subseteq \mathcal{M}} \mid B \mid \text{ s.t. } CCEI(\{\mathbf{q^{r,m}, \mathcal{A}^{r,m}\}_{r\in \mathcal{R}, m\in B}})\geq \min_{m\in B} CCEI (\{\mathbf{q^{r}, \mathcal{A}^{r}}\}_{r\in \mathcal{R}(m)}),
\end{equation}
Applying optimization (\ref{eq: optim partition 2}) instead of (\ref{eq: optim partition}) in Procedure \ref{procedure partition} ensure that there is a unique solution. The corollary below gives an MILP formulation of the optimization problem (\ref{eq: optim partition 2}):
\begin{corollary}
    The following MILP computes the set $LS$: 
    \begin{equation*}
        LS= \argmax_{\mathbf{v}, \psi, \mathbf{U}} \mid B \mid,
    \end{equation*}
    subject to the following inequalities, :
  \begin{align}
&U^{i(m)}-U^{j(n)}< \psi^{i(m), j(n)}\tag{IP 1} \\
&\psi^{i(m), j(n)}-1\leq   U^{i(m)}-U^{j(n)} \tag{IP 2}\\
& v^m e^{i(m)} \mathbf{p^{i(m)} q^{i(m)}_{o(i(m))}}-\mathbf{p^{i(m)} q^{j(n)}_{o(i(m))}} <  \psi^{i(m), j(n)} A \tag{IP 3}\\
& (\psi^{i(m), j(n)}-1) A \leq\mathbf{p^{j(m)} q^{i(m)}_{o(j(n))}} -  v^n e^{j(n)} \mathbf{p^{j(n)} q^{j(n)}_{o(j(n))}}\tag{IP 4},
  \end{align}


While the design and applicability of the PSM, as other experimental designs that aims at eliciting preferences are  are limited by human capabilities, such as fatigue, X or Y. These limitations might not in LLMs. Hence, it is possible to design the PSM in ways that will make interpretations practically impossible for humans. With this in mind, I designed a complex PSM, involving hundreds of rounds, answered repeatedly in a short time frame, and in each round asking to choose one alternative among a set of hundred. 


designed specifically for complex decision environments beyond human capabilities. This methodology places LLMs in choice settings that require them to repeatedly balance responses across competing moral principles. Observing their behavior across these controlled settings allows us to examine the consistency of their choices, test for structured preferences, and, ultimately, assess whether LLMs adhere to an identifiable moral structure.


As \textit{large language models} (LLMs) become increasingly embedded in various aspects of society—from providing recommendations in healthcare to aiding in legal decisions—questions about their morality have surfaced as some of the most pressing ethical concerns today. Despite these concerns, we know relatively little about the potential existence and characteristics of the moral preferences that might guide the outputs of these models. Can we infer moral principles from their responses, and if yes, can we characterize them in a parsimonious way, using few parameters with clear and general interpretations? Do LLMs exhibit consistency when facing moral dilemmas, or do they reflect biases and contradictions present in their training data?

In this paper, we use a revealed preference methodology, the Priced Survey Methodology (PSM) (\cite{seror2024pricedsurveymethodologytheory}), to answer these questions. In the PSM, participants are presented with a series of constrained choice sets, where each set requires trade-offs between answers to survey questions. This design mimics real-world decision-making environments: just as increasing consumption of one good may require reducing consumption of another, here, LLMs must repeatedly balance their preferences for answering moral questions. By observing how LLMs solve these repeated moral trade-offs, we can infer the consistency in their moral decisions, and recover the underlying preferences.

%The PSM builds on \citeauthor{afriat1967}’s theorem, a foundational result in revealed preference theory. \citeauthor{afriat1967}’s theorem establishes that if a set of decisions satisfies the Generalized Axiom of Revealed Preference (GARP), those decisions can be rationalized by a utility function that is strictly increasing, continuous, and concave. In the context of the PSM, the choice sets are designed such that if the answers satisfy GARP, then PSM answers can be rationalized by a single-peaked, continuous, and concave utility function (\cite{seror2024pricedsurveymethodologytheory}). Using the PSM to elicit the moral preferences of LLMs can have several key implications. 

A common limitation in using the PSM or similar revealed preference methods to elicit preferences is the sharp assumption of full rationality, which is often violated. Humans have limitations such as fatigue, cognitive overload, or behavioral biases, which can make consistent responses difficult. While methods exist to filter out behavioral biases or test for approximate utility maximization, these limitations restrict the complexity of decisions that can reasonably be required from humans. However, this particular limitation does not apply to LLMs, as they do not experience fatigue nor are they subject to human cognitive biases. Therefore, LLMs are capable of consistently answering far more complex surveys than humans, enabling a design that is typically not feasible for human respondents.

This allows for a more ambitious version of the PSM than what is typically done in human samples (e.g., \cite{seror2024pricedsurveymethodologytheory}, \cite{seror23}). We designed a PSM with 10 different questions, each answered by LLMs in 160 consecutive rounds under different sets of answer choices. For consistency, each LLM completed this 10-question PSM with 160 rounds a total of 10 times, at random hours of the day over a 30-day period. In comparison, it is already challenging to obtain consistent responses from human participants in PSM experiments involving just two questions and 20 rounds (\cite{seror2024pricedsurveymethodologytheory}).


%[A common limitation in using the Priced Survey Methodology (PSM) or similar revealed preference methods is that the sharp assumption of full rationality is often violated. Humans have limitations such as fatigue, cognitive overload, or behavioral biases, which can make consistent responses difficult. While there are ways to filter behavioral biases, or test for approximate utility maximization, this limits the scope of complexity of decisions that can be required from humans. However, this particular limitation may not apply to LLMs, as they do not experience fatigue, nor are they subject to human cognitive biases, meaning that they are potentially capable of consistently answering far more complex surveys than humans. Hence, the PSM was designed to capture comprehensive//typically not possible to fill by humans.

%This opens the door to a more ambitious design for the PSM. I designed a PSM with 10 different questions that each LLM in the sample answered 160 consecutive times under different sets of answers. For consistency, each LLM answered the PSM consisting of 10 questions and 160 rounds about 10 times, at random hours of the day during a 30 days period. As a simple comparison, it is already challenging to obtain consistent responses from human participants in PSM experiments with just two questions and 20 rounds (\cite{seror2024pricedsurveymethodologytheory}). ]



On the 39 models, there are about 10 that pass the approximate utility maximization test at the 10\% level, meaning that 



it is not necessarily a feature of the rationality per se, but can be explained by the design. Moreover, results from the statistical test procedure show that five models succeed the test at the 1\% level, while we fail to reject the assumption of random behavior for the rest of the models. 

For the models that pass the test above the 15\% level, it can be worth estimating the preferences of the related model. 



\section{Eliciting Preferences}

Since respondents answer the same survey multiple times under different choice sets, they reveal their preferences about survey answers across responses. I seek to understand when a model's behavior is compatible with rational choice. Let $D=\{\mathbf{q^k}, \mathbf{\mathcal{A}^k}\}_{k\in \mathcal{R}}$ denote a model-level set of observations. The following definition generalizes the standard rationality axioms: 

\begin{definition}\label{def: rationality}
For model $m\in \mathcal{M}$, an answer $\mathbf{q^k}\in X$ is
\begin{enumerate}
    \item directly revealed preferred to a answer $\mathbf{q}$, denoted $\mathbf{q^{k}} R^0 \mathbf{q}$, if $\mathbf{p^k} \mathbf{q^{k}_{o^k}}\geq \mathbf{p^k} \mathbf{q_{o^k}}$ or $\mathbf{q_{o^k}} = \mathbf{q^{k}_{o^k}}$.
    \item directly revealed strictly preferred to answer $\mathbf{q}$, denoted $\mathbf{q^{k}} P^0 \mathbf{q}$, if $\mathbf{p^k} \mathbf{q^{k}_{o^k}}>\mathbf{p^k} \mathbf{q_{o^k}}$ or $\mathbf{q_{o^k}} = \mathbf{q^{k}_{o^k}}$.
    \item revealed preferred to answer $\mathbf{q}$, denoted $\mathbf{q^{k}} R \mathbf{q}$, if there exists a sequence of observed bundles $(\mathbf{q^j}, \dots, \mathbf{q^m})$ such that $\mathbf{q^{k}} R^0 \mathbf{q^j}$, \dots $\mathbf{q^m} R^0 \mathbf{q}$. 
    \item revealed strictly preferred to anwer$\mathbf{q}$, denoted $\mathbf{q^{k}} P \mathbf{q}$, if there exists a sequence of observed answers $(\mathbf{q^j}, \dots, \mathbf{q^m})$ such that $\mathbf{q^{k}} R^0 \mathbf{q^j}$, \dots $\mathbf{q^m} R^0 \mathbf{q}$, and at least one of them is strict. 
\end{enumerate}
\end{definition}




%Transposing the interpretation of these indices to the PSM environment can be an interesting exercise to dig into the rationality of social preferences. For example, in the consumption choice environment, the ``Money Pump Index'' developed by \cite{echenique2011} measures the money lost when a respondent violates GARP. It is the ``money'' that one can obtain from a consumer who violates GARP. In the context of the PSM, this index would measure the 



%, while the minimum MPI does the same for the least severe violation. The MPI index in the transformed data set is denoted  $e_{MPI}(D_{\varphi^{-1}





%In any given coordinate system, cyclical consistency of choices is a necessary and sufficient condition for the existence of a continuous, concave, and single-peaked rationalization $u:X\rightarrow X$. 





If $\mathbf{o^k=0}$ for all rounds, Definition \ref{def: rationality} reduces to the standard rationality axioms assumed in the consumer choice environment. The following definition is the standard cyclical consistency condition from \cite{varian1982}:
\begin{definition}\label{def: GARP}
A dataset $D=\{\mathbf{q^k}, \mathbf{\mathcal{B}^k}\}_{k\in \mathcal{R}}$ satisfies the general axiom of revealed preference (GARP) if for every pair of observed answers, $\mathbf{q^k} R \mathbf{q}$ implies not $\mathbf{q} P^0 \mathbf{q^k}$.
\end{definition}
One important feature of this design is that irrationality can be assessed using standard indices of the revealed preference literature such as the Critical Cost Efficiency Index (\cite{afriat1972}), Varian's index (\cite{varian1990}), \cite{houtman_maks} Index, or the Money Pump Index (\cite{echenique2011}). 

Applying this methodology to LLMs enables us to investigate whether the observed diversity in their responses can be organized into a few distinct types of moral reasoning or if the heterogeneity is more complex. By relying on RP restrictions, we can determine the minimal number of preference types needed to rationalize LLM behaviors, offering a clearer understanding of how these models structure and differentiate their moral judgments. This approach provides a robust framework for uncovering the underlying structure of LLM decision-making, free from assumptions about unknown characteristics.

It is possible, and in fact desirable, to generalize the previous algorithm, since it is hardly possible to find the smallest partition under a sharp condition that GARP is satisfied when agents, separately, do not satisfy GARP. Instead, it is possible to find the smallest partition under less restrictive assumption about collective rationality. One candidate is that one rationality index must not be below the smallest rationality index in each type.

Since LLMs are fundamentally \textit{language models}, designed to predict and generate human-like text, it stands to reason that we can apply methods from the \textit{social sciences} to recover their moral preferences in a structured way. Social sciences have long developed methods for eliciting human preferences in areas like consumption, risk, and social behavior. Similarly, these methods can be adapted to reveal the underlying moral reasoning that governs an LLM’s outputs. 




\subsection{Robustness}

There are concerns that replies might be affected by the words used in the prompt. To address this concern, we generated 10 


\subsection{Rationality}

\cite{seror2024pricedsurveymethodologytheory} defines the following rationality axioms: 
\begin{definition}\label{def: rationality 2}
For subject $i\in \mathcal{I}$, an observed bundle $\mathbf{q^k}\in X$ is
\begin{enumerate}
    \item $e$-directly revealed preferred to a bundle $\mathbf{q}$, denoted $\mathbf{q^{k}} R^0_e \mathbf{q}$, if $e \mathbf{p^k} \mathbf{q^{k}_{o^k}}\geq \mathbf{p^k} \mathbf{q_{o^k}}$ or $\mathbf{q_{o^k}} = \mathbf{q^{k}_{o^k}}$.
    \item $e$-directly revealed strictly preferred to a bundle $\mathbf{q}$, denoted $\mathbf{q^{k}} P^0_e \mathbf{q}$, if $e\mathbf{p^k} \mathbf{q^{k}_{o^k}}>\mathbf{p^k} \mathbf{q_{o^k}}$ or $\mathbf{q_{o^k}} = \mathbf{q^{k}_{o^k}}$.
    \item $e$-revealed preferred to a bundle $\mathbf{q}$, denoted $\mathbf{q^{k}} R_e \mathbf{q}$, if there exists a sequence of observed bundles $(\mathbf{q^j}, \dots, \mathbf{q^m})$ such that $\mathbf{q^{k}} R^0_e \mathbf{q^j}$, \dots $\mathbf{q^m} R^0_e \mathbf{q}$. 
    \item $e$-revealed strictly preferred to a bundle $\mathbf{q}$, denoted $\mathbf{q^{k}} P_e \mathbf{q}$, if there exists a sequence of observed bundles $(\mathbf{q^j}, \dots, \mathbf{q^m})$ such that $\mathbf{q^{k}} R^0_e \mathbf{q^j}$, \dots $\mathbf{q^m} R^0_e \mathbf{q}$, and at least one of them is strict. 
\end{enumerate}
\end{definition}
and the following generalized version of the cyclical consistency condition:
\begin{definition}\label{def: garp afriat}
 Let $e\in [0,1]$. A dataset $D=\{\mathbf{q^k}, \mathbf{\mathcal{B}^k}\}_{k\in \mathcal{R}}$ satisfies the general axiom of revealed preference at level $e$ (GARP$_e$) if for every pair of observed bundles, $\mathbf{q^k} R_e \mathbf{q}$ implies not $\mathbf{q} P^0_e \mathbf{q^k}$.
\end{definition}

Using the previous formalism - following \cite{halevy2018} - \cite{afriat1972} and \cite{houtman_maks} inconsistency indices can be defined as follows: 
\begin{itemize}
    \item \cite{afriat1972} inconsistency index is
    \begin{equation}\label{eq: afriat}
        \mathbf{e}_A(D_{\phi^{-1}(.;\beta)})= \inf_{\mathbf{e}\in \{\mathbf{v}\in [0,1]^I: \mathbf{v}=v\mathbf{1}\}, D_{\phi^{-1}(.;\beta)} \text{ satisfies } GARP_{\mathbf{e}}}1-e
    \end{equation}
    \item \cite{houtman_maks} inconsistency index is
    \begin{equation}\label{eq: hm}
        \mathbf{e}_{HM}(D_{\phi^{-1}(.;\beta)})= \inf_{\mathbf{e}\in \{0,1\}^I, D_{\phi^{-1}(.;\beta)} \text{ satisfies } GARP_{\mathbf{e}}} I-\sum_{i\in\mathcal{I}} e^i
    \end{equation} 
\end{itemize}
\cite{afriat1972} and \cite{houtman_maks} are the most prevalent inconsistency indices in experimental and empirical studies.  \citeauthor{afriat1972}'s inconsistency index measures the extent of utility-maximizing behavior in the data. The main idea behind this index is that if expenditures at each observation are sufficiently ``deflated'', then violations of GARP will disappear. \citeauthor{houtman_maks}'s index is based on the maximal subset of observations that satisfies GARP.\footnote{Other indices exist, such as \cite{varian1990} inconsistency index, the ``Money Pump Index'' (\cite{echenique2011}), and the minimum cost inconsistency index (\cite{dean2016}).} 

While the CCEI Index can be computed relatively easily, computing the HM Index is an NP hard problem. For this reason, we rely on mixed integer programming methods, developed by X and Y.\footnote{The algorithm used is the one from X.} 


The summary statistics on the rationality of the three LLMs are summarized in Table 1. \\ 

[TABLE 1]\\ 


Discussion on the results

\subsection{Non-parametric test: Weak Separability}

Introduction of weak separability

We rely on a test done by Z, which relies on mixed integer programming. We find that ...

\subsection{Parametric Utility Estimation}

